Microfluidics Generation of Millimeter-sized Matrigel Droplets

Significant progress has been made to increase access to droplet microfluidics for labs with limited microfluidics expertise or fabrication equipment. In particular, using off-the-shelf systems has been a valuable approach. However, the ability to modify a channel design and, thus, the functional characteristics of the system is of great value. In this work, we describe the development of co-flow microfluidics and their fabrication methods for generating uniform millimeter-sized (0.5 - 2 mm) hydrogel droplets. Two complementary approaches based on desktop CO2 laser cutting were developed to prototype and build durable co-flow droplet microfluidics. After demonstrating the co-flow systems, water-in-oil experiments and dimensionless number analysis were used to examine the operational characteristics of the system. Specifically, the Capillary number analysis indicated that millimeter-sized droplet generators operated in the desirable geometry-controlled regime despite their length scales being larger than traditional microfluidics systems. Next, the tunable generation of Matrigel droplets was demonstrated. By adjusting the relative flow rates, the droplet size could be tuned. Finally, we demonstrated fibroblast encapsulation and cell viability for up to 7 days as a proof-of-concept experiment. The systems presented are simple and effective tools to generate robust hydrogel droplets and increase the accessibility of this technology to teaching labs or research settings with limited resources or access to microfluidics.

==> refs.tex <==
@article{teh2008droplet,
  title={Droplet microfluidics},
  author={Teh, Shia-Yen and Lin, Robert and Hung, Lung-Hsin and Lee, Abraham P},
  journal={Lab on a Chip},
  volume={8},
  number={2},
  pages={198--220},
  year={2008},
  publisher={Royal Society of Chemistry}
}

@article{chen2022trends,
  title={Trends in droplet microfluidics: from droplet generation to biomedical applications},
  author={Chen, Zhengkun and Kheiri, Sina and Young, Edmond WK and Kumacheva, Eugenia},
  journal={Langmuir},
  volume={38},
  number={20},
  pages={6233--6248},
  year={2022},
  publisher={ACS Publications}
}

@article{klein2015droplet,
  title={Droplet barcoding for single-cell transcriptomics applied to embryonic stem cells},
  author={Klein, Allon M and Mazutis, Linas and Akartuna, Ilke and Tallapragada, Naren and Veres, Adrian and Li, Victor and Peshkin, Leonid and Weitz, David A and Kirschner, Marc W},
  journal={Cell},
  volume={161},
  number={5},
  pages={1187--1201},
  year={2015},
  publisher={Elsevier}
}

@article{brower2020double,
  title={Double emulsion flow cytometry with high-throughput single droplet isolation and nucleic acid recovery},
  author={Brower, Kara K and Carswell-Crumpton, Catherine and Klemm, Sandy and Cruz, Bianca and Kim, Gaeun and Calhoun, Suzanne GK and Nichols, Lisa and Fordyce, Polly M},
  journal={Lab on a Chip},
  volume={20},
  number={12},
  pages={2062--2074},
  year={2020},
  publisher={Royal Society of Chemistry}
}

@article{iyer2022advancing,
  title={Advancing microfluidic diagnostic chips into clinical use: a review of current challenges and opportunities},
  author={Iyer, Vasant and Yang, Zijian and Ko, Jina and Weissleder, Ralph and Issadore, David},
  journal={Lab on a Chip},
  year={2022},
  publisher={Royal Society of Chemistry}
}

@article{agresti2010ultrahigh,
  title={Ultrahigh-throughput screening in drop-based microfluidics for directed evolution},
  author={Agresti, Jeremy J and Antipov, Eugene and Abate, Adam R and Ahn, Keunho and Rowat, Amy C and Baret, Jean-Christophe and Marquez, Manuel and Klibanov, Alexander M and Griffiths, Andrew D and Weitz, David A},
  journal={Proceedings of the National Academy of Sciences},
  volume={107},
  number={9},
  pages={4004--4009},
  year={2010},
  publisher={National Acad Sciences}
}

@article{price2016discovery,
  title={Discovery in droplets},
  author={Price, Alexander K and Paegel, Brian M},
  journal={Analytical chemistry},
  volume={88},
  number={1},
  pages={339--353},
  year={2016},
  publisher={ACS Publications}
}

@article{postek2017precise,
  title={A precise and accurate microfluidic droplet dilutor},
  author={Postek, W and Kaminski, TS and Garstecki, P},
  journal={Analyst},
  volume={142},
  number={16},
  pages={2901--2911},
  year={2017},
  publisher={Royal Society of Chemistry}
}

@article{werner2022phase,
  title={Phase-Optimized Peristaltic Pumping by Integrated Microfluidic Logic},
  author={Werner, Erik M and Lam, Benjamin X and Hui, Elliot E},
  journal={Micromachines},
  volume={13},
  number={10},
  pages={1784},
  year={2022},
  publisher={MDPI}
}

@article{prakash2007microfluidic,
  title={Microfluidic bubble logic},
  author={Prakash, Manu and Gershenfeld, Neil},
  journal={Science},
  volume={315},
  number={5813},
  pages={832--835},
  year={2007},
  publisher={American Association for the Advancement of Science}
}

@article{tan2007monodisperse,
  title={Monodisperse alginate hydrogel microbeads for cell encapsulation},
  author={Tan, W-H and Takeuchi, Shoji},
  journal={Advanced materials},
  volume={19},
  number={18},
  pages={2696--2701},
  year={2007},
  publisher={Wiley Online Library}
}
@article{trivedi2010modular,
  title={A modular approach for the generation, storage, mixing, and detection of droplet libraries for high throughput screening},
  author={Trivedi, Varun and Doshi, Ankur and Kurup, GK and Ereifej, E and Vandevord, PJ and Basu, Amar S},
  journal={Lab on a Chip},
  volume={10},
  number={18},
  pages={2433--2442},
  year={2010},
  publisher={Royal Society of Chemistry}
}

@article{agarwal2017microfluidics,
  title={Microfluidics enabled bottom-up engineering of 3D vascularized tumor for drug discovery},
  author={Agarwal, Pranay and Wang, Hai and Sun, Mingrui and Xu, Jiangsheng and Zhao, Shuting and Liu, Zhenguo and Gooch, Keith J and Zhao, Yi and Lu, Xiongbin and He, Xiaoming},
  journal={ACS nano},
  volume={11},
  number={7},
  pages={6691--6702},
  year={2017},
  publisher={ACS Publications}
}

@article{shao2022user,
  title={User-friendly microfluidic manufacturing of hydrogel microspheres with sharp needle},
  author={Shao, Lei and Pan, Bingchu and Hou, Ruxia and Jin, Yuan and Yao, Yudong},
  journal={Biofabrication},
  volume={14},
  number={2},
  pages={025017},
  year={2022},
  publisher={IOP Publishing}
}

@article{zhang2022one,
  title={One-step generation and purification of cell-encapsulated hydrogel microsphere with an easily assembled microfluidic device},
  author={Zhang, Tao and Zhang, Hong and Zhou, Wuping and Jiang, Keming and Liu, Cong and Wang, Ru and Zhou, Yuanshuai and Zhang, Zhiqiang and Mei, Qian and Dong, Wen-Fei and others},
  journal={Frontiers in Bioengineering and Biotechnology},
  volume={9},
  pages={1504},
  year={2022},
  publisher={Frontiers}
}

@article{dolega2015controlled,
  title={Controlled 3D culture in Matrigel microbeads to analyze clonal acinar development},
  author={Dolega, Monika E and Abeille, Fabien and Picollet-d'Hahan, Nathalie and Gidrol, Xavier},
  journal={Biomaterials},
  volume={52},
  pages={347--357},
  year={2015},
  publisher={Elsevier}
}

@article{zhang2021microfluidic,
  title={Microfluidic droplets as structural templates for Matrigel to enable 1-week large organoid modeling},
  author={Zhang, Weijie and Li, Donghui and Jiang, Shengwei and Galan, Edgar A and Zhang, Zhongyue and Huang, Laiqiang and Ma, Shaohua},
  journal={Chemical Engineering Science},
  volume={238},
  pages={116632},
  year={2021},
  publisher={Elsevier}
}

@article{wu2020rapid,
  title={Rapid microfluidic formation of uniform patient-derived breast tumor spheroids},
  author={Wu, Zhuhao and Gong, Zhiyi and Ao, Zheng and Xu, Junhua and Cai, Hongwei and Muhsen, Maram and Heaps, Samuel and Bondesson, Maria and Guo, Shishang and Guo, Feng},
  journal={ACS Applied Bio Materials},
  volume={3},
  number={9},
  pages={6273--6283},
  year={2020},
  publisher={ACS Publications}
}

@article{wang2023recent,
  title={Recent methods of droplet microfluidics and their applications in spheroids and organoids},
  author={Wang, Yihe and Liu, Mengqi and Zhang, Yu and Liu, Hong and Han, Lin},
  journal={Lab on a Chip},
  year={2023},
  publisher={Royal Society of Chemistry}
}

@article{lashkaripour2018desktop,
  title={Desktop micromilled microfluidics},
  author={Lashkaripour, Ali and Silva, Ryan and Densmore, Douglas},
  journal={Microfluidics and Nanofluidics},
  volume={22},
  pages={1--13},
  year={2018},
  publisher={Springer}
}

@article{hassani2022developing,
  title={Developing an Off-the-Shelf Microfluidic Droplet Generation Device for Cell Encapsulation},
  author={Hassani-Gangaraj, Mojtaba and Shamloo, Amir},
  journal={Industrial \& Engineering Chemistry Research},
  volume={61},
  number={30},
  pages={10689--10699},
  year={2022},
  publisher={ACS Publications}
}

@article{anna2016droplets,
  title={Droplets and bubbles in microfluidic devices},
  author={Anna, Shelley Lynn},
  journal={Annual Review of Fluid Mechanics},
  volume={48},
  pages={285--309},
  year={2016},
  publisher={Annual Reviews}
}

@article{thompson2013adhesive,
  title={Adhesive-based bonding technique for PDMS microfluidic devices},
  author={Thompson, C Shea and Abate, Adam R},
  journal={Lab on a Chip},
  volume={13},
  number={4},
  pages={632--635},
  year={2013},
  publisher={Royal Society of Chemistry}
}

@article{jeyasountharan2023viscoelastic,
  title={Viscoelastic Particle Encapsulation Using a Hyaluronic Acid Solution in a T-Junction Microfluidic Device},
  author={Jeyasountharan, Anoshanth and Giudice, Francesco Del},
  journal={Micromachines},
  volume={14},
  number={3},
  pages={563},
  year={2023},
  publisher={MDPI}
}
@article{rojek2022microfluidic,
  title={Microfluidic Formulation of Topological Hydrogels for Microtissue Engineering},
  author={Rojek, Katarzyna O and Cwiklinska, Monika and Kuczak, Julia and Guzowski, Jan},
  journal={Chemical Reviews},
  volume={122},
  number={22},
  pages={16839--16909},
  year={2022},
  publisher={ACS Publications}
}

@misc{Labno_cell_count,
    author= {Christine Labno},
    title = {Two Ways to Count Cells with ImageJ},
    note  = {\url{https://www.unige.ch/medecine/bioimaging/files/3714/1208/5964/CellCounting.pdf}, 
             Last accessed on 2023-05-10},
}

